Low-Rank Quantization-Aware Training for LLMs

Large language models (LLMs) are omnipresent, however their practical deployment is challenging due to their ever increasing computational and memory demands. Quantization is one of the most effective ways to make them more compute and memory efficient. Quantization-aware training (QAT) methods, generally produce the best quantized performance, however it comes at the cost of potentially long training time and excessive memory usage, making it impractical when applying for LLMs. Inspired by parameter-efficient fine-tuning (PEFT) and low-rank adaptation (LoRA) literature, we propose LR-QAT -- a lightweight and memory-efficient QAT algorithm for LLMs. LR-QAT employs several components to save memory without sacrificing predictive performance: (a) low-rank auxiliary weights that are aware of the quantization grid; (b) a downcasting operator using fixed-point or double-packed integers and (c) checkpointing. Unlike most related work, our method (i) is inference-efficient, leading to no additional overhead compared to traditional PTQ; (ii) can be seen as a general extended pretraining framework, meaning that the resulting model can still be utilized for any downstream task afterwards; (iii) can be applied across a wide range of quantization settings, such as different choices quantization granularity, activation quantization, and seamlessly combined with many PTQ techniques. We apply LR-QAT to LLaMA-1/2/3 and Mistral model families and validate its effectiveness on several downstream tasks. Our method outperforms common post-training quantization (PTQ) approaches and reaches the same model performance as full-model QAT at the fraction of its memory usage. Specifically, we can train a 7B LLM on a single consumer grade GPU with 24GB of memory. Our source code is available at https://github.com/qualcomm-ai-research/LR-QAT

==> figures/04_ablation_rank.tex <==
% 
\begin{figure*}[tb]
    % \vspace{-.2cm}
    \includegraphics[width=0.5\textwidth]{img/04_ablation_rank.png}
    \caption{The performance of {\method} ($\dcfn{} = {\text{\nf{Q4.4}}}$) depending on the rank $r$ of auxiliary matrices $\A$ and $\B$ on {\llama}-2 7B with W4 per-channel quantization.}
    \label{fig:04_ablation_rank}
\end{figure*}
% 

==> figures/_archive/03_fixed_point8.tex <==
% 
% 
\begin{figure*}[tb]
    % \vspace{-.2cm}
    \includegraphics[width=.4\textwidth]{img/03_fixed_point8.png}
    \caption{An overview of FixedPoint8 numeric format.}
    \label{fig:03_fixed_point8}
\end{figure*}
% 
% 

==> figures/_archive/03_lora_qat.tex <==
% 
\begin{figure*}[tb]
    % \vspace{-.2cm}
    \includegraphics[width=.7\textwidth]{img/03_lora_qat.png}
    \caption{Our proposed method.}
    \label{fig:03_lora_qat}
\end{figure*}
% 

==> figures/_archive/03_memory_breakdown.tex <==
% 
\begin{figure*}[tb]
\subfloat[Vanilla QAT / fine-tuning]{
    \includegraphics[width=.5\textwidth]{img/03_memory_breakdown_vanilla.png}
}
\subfloat[LoRa-QAT]{
    \includegraphics[width=.5\textwidth]{img/03_memory_breakdown_lora_qat.png}
}
%
\centering
% \vspace{-.15cm}
\caption{%
Memory breakdown.
}
\label{fig:03_memory_breakdown}
\end{figure*}
% 

==> figures/_archive/04_init_ablation_opt.tex <==
% 
\begin{figure*}[tb]
    % \vspace{-.2cm}
    \includegraphics[width=\textwidth]{img/04_init_ablation_opt.png}
    \caption{Ablation study on LoRA adapters initialization on OPT-1.3B.}
    \label{fig:04_init_ablation_opt}
\end{figure*}
% 

==> figures/rebuttal_upd_mem.tex <==
\begin{figure}[tp]
    \centering
        % \centering
        % \includegraphics[width=0.4\textwidth]{img/01_lora_qat.png}
        % \hspace{0.03\textwidth}
        % \centering
        % \raisebox{0.01\height}{\includegraphics[width=0.48\textwidth]{img/memory_plot_original_palette.png}}
        % \hspace{0.01\textwidth}

        % \centering
        % \includegraphics[width=0.4\textwidth]{img/01_lora_qat_proposed_palette.png}
        % \includegraphics[width=0.375\textwidth]{img/01_lora_qat_yell.png}
        % \hspace{0.03\textwidth}
        % \centering
        % \raisebox{0.01\height}{\includegraphics[width=0.48\textwidth]{img/memory_plot_proposed_palette.png}}
        \raisebox{-0.04\height}{\includegraphics[width=0.555\textwidth]{img/01_memory_plot_yell.png}}
        \hspace{0.01\textwidth
        }   
    \caption{Memory requirements for training with various QAT techniques on {\llama}-2 7B, assuming batch size 1, sequence length 1024, $r=32$, and {\nf{BF16}} compute data type.
    % 
    `Intermediate results' refer to the results of some intermediate computations, \eg{} after rounding/clipping, which are saved in memory for the backward pass.
    }     %\vspace{-0.4cm}
    \label{fig:new_fig_one}
    \vspace{-.2cm}
\end{figure}



==> tables/_archive/04_2_bit_results.tex <==
% 
%
\begin{table*}[tb]
    \setlength{\tabcolsep}{8pt}
    \centering
    \caption{\u{2-bit weight quantization results for {\llama}-2 7B}. 
    We report WikiText-2 test set perplexity and average zero-shot accuracy. Numbers marked in bold are SOTA. {\ts{\S}}Uses asymmetric weight quantization.}
    \label{tbl:04_2_bit_results}
    \resizebox{0.65\columnwidth}{!}{%
    \begin{tabular}{ lcccc }
        \toprule
        % 
        \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{WikiText-2 perplexity $\da$} & \multicolumn{2}{c}{Zero-shot accuracy $\ua$} \\[0.1em]
        & W2\,pc & W2\,g128 & W2\,pc & W2\,g128 \\
        % 
        \midrule
        % 
        FP16 & \multicolumn{2}{c}{5.68} & \multicolumn{2}{c}{69.68} \\
        \midrule
        RTN\ts{\S} & 5.2e3 & 2.5e3 & 36.52 & 37.94 \\
        GPTQ\ts{\S} & 7.7e3 & 36.77 & - & - \\
        AWQ & - & 2.2e5 & - & - \\
        OmniQuant\ts{\S} & 37.37 & 11.06 & - & - \\
        PEQA (our impl.)\ts{\S} & 9.34 & {7.87} & 57.40 & {60.74} \\
        \gcb{\method{} (ours)}\ts{\S} & \gcb{8.51} & \gcb{7.62} & \gcb{60.03} & \gcb{61.70} \\
        % 
        \bottomrule
    \end{tabular}
        % \vspace{-.15cm}
    }  % end resizebox
    \vspace{-.2cm}
\end{table*}
% 



==> tables/_archive/04_ablation_dtype_init.tex <==
% 
%
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    \centering
    \caption{The performance of {\method} applied to {\llama}-2 7B depending on the choice of downcasting operator $\dcfn\p{\cdot}$, compute data type and initialization method for low-rank auxiliary matrices.}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{ lllcccc }
            \toprule
            % 
            \multirow{2}{*}{$\dcfn\p{\cdot}$} & \multirow{2}{*}{dtype} & \multirow{2}{*}{$\A$, $\B$ init.} & \multicolumn{2}{c}{W4pc} & \multicolumn{2}{c}{W3pc} \\[0.25em]
            & & & WikiText-2 $\da$ & Zero-shot acc. $\ua$ & WikiText-2 $\da$ & Zero-shot acc. $\ua$  \\
            % 
            \midrule
            % 
            {\nf{FP32}} & {\nf{FP32}} & LoRA & 5.69 & 69.28 & 6.21 & 66.62 \\
            \midrule
            {\nf{FP16}} & {\nf{FP32}} & LoRA & $+$0.00 & $-$0.13 & $+$0.01 & $-$0.01 \\
            {\nf{BF16}} & {\nf{FP32}} & LoRA & $-$0.01 & $+$0.11 & $+$0.01 & $+$0.45 \\
            {\nf{Q4.4} / \nf{Q3.5}} & {\nf{FP32}} & LoRA & $-$0.01 & $+$0.16 & $+$0.01 & $+$0.31 \\
            \u{\nf{Q4.4} / \nf{Q3.5}} & \u{\nf{BF16}} & \u{LoRA} & \u{$-$0.01} & \u{$+$0.15} & \u{$+$0.01} & \u{$+$0.31} \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoRA & $+$0.02 & $-$0.04 & $+$1.5e3 & $-$30.30 \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoftQ ($T=1$) & $+$0.14 & $-$1.02 & $+$0.18 & $+$0.26 \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoftQ ($T=64$) & $+$0.40 & $-$1.40 & $+$1.37 & $-$2.01 \\
            % 
            \bottomrule
        \end{tabular}
        % \vspace{-.15cm}
    }  % end resizebox
    \label{tbl:04_ablation_dtype_init}
\end{table*}
% 


==> tables/_archive/04_memory_usage.tex <==
% 
%
\begin{table*}[htb]
    \centering
    \begin{tabular}{ cccc }
        \toprule
         Method $r$ & WikiText-2 Perplexity $\da$ & Zero-shot avg. accuracy $\ua$ & CUDA memory used, GB \\
         \midrule  
         FP16 & 0 & 0 & 0 \\
         \midrule  
         Naive PTQ & 0 & 0 & 0 \\
         Scales only QAT & 0 & 0 & 0 \\
         Full-model QAT & 0 & 0 & 0 \\
         \gcb{LoRa-QAT} & \gcb{0} & \gcb{0} & \gcb{0} \\
         \gcb{LoRa-QAT} & \gcb{0} & \gcb{0} & \gcb{0} \\
         \gcb{LoRa-QAT} & \gcb{0} & \gcb{0} & \gcb{0} \\
         \bottomrule
    \end{tabular}
    % \vspace{-.15cm}
    \caption{
    Comparison of memory usage.
}
    \label{tbl:04_memory_usage}
\end{table*}
% 


==> tables/_archive/04_weight_act_quant_results_OLD.tex <==
\begin{table*}[t]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{Weight and activation quantization results for {\llama}-1 7B}. 
    We report WikiText-2 test set perplexity (lower is better) and zero-shot accuracy of 6 tasks (higher is better). Numbers marked in bold are SOTA. {\ts{\S}}Uses asymmetric weight quantization. {\ts{*}}Uses a maximum sequence length of 1024 for evaluation.}
    \label{tbl:04_weight_act_quant_results}
    \renewcommand{\arraystretch}{1.0}
    % 
    \resizebox{1.0\columnwidth}{!}{%
        \begin{tabular}{clcccccccc}
            \toprule
            \multirow{2}{*}{\begin{tabular}{c}\# Bits\\(W-A-KV)\end{tabular}} & \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multirow{2}{*}{WikiText-2 $\da$} & \multicolumn{7}{c}{Zero-shot accuracy $\ua$} \\[0.25em]
            & & & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & \u{Avg.} \\
            \midrule
            %
            % 
            FP16 & & 5.68 & 75.05 & 79.16 & 70.01 & 72.85 & 44.80 & 76.21 & 69.68 \\
            \midrule
            %
            % 
            % \multirow{2}{*}{\shortstack{4/16/16}} 
            % & RTN, min-max & 6.85 & 71.19 & 77.42 & 67.17 & 66.92 & 42.49 & 72.16 & 66.23 \\
            % & RTN, best & 6.33 & 74.40 & 77.86 & 68.75 & 71.42 & 44.11 & 74.79 & 68.56 \\
            % \midrule
            %
            % 
            \multirow{4}{*}{\shortstack{4-8-8}} 
            & RTN & 6.88 & 71.35 & 76.66 & 66.46 & 66.84 & 41.55 & 72.10 & 65.83 \\
            & SmoothQuant & 13.7\ts{*} & 71.00 & 76.00 & 66.00 & 67.40 & 42.80 & 67.80 & 65.17 \\
            & LLM-QAT & 11.2\ts{*} & 74.60 & 77.50 & 67.70 & 70.20 & \u{45.60} & 73.50 & {68.18} \\
            & PEQA (our impl.) & 5.89 & \u{74.86} & 78.24 & 70.01 & 70.12 & 42.83 & \u{75.14} & 68.53 \\
            & \gcb{LR-QAT (ours)} & \gcb{5.85} & \gc{73.76} & \gcb{78.51} & \gcb{71.19} & \gcb{71.09} & \gc{41.81} & \gc{75.10} & \gcb{68.58} \\
            \midrule
            %
            %
            \multirow{5}{*}{\shortstack{4-8-4}} 
            & RTN & 7.66 & 68.81 & 75.46 & 62.12 & 62.46 & 39.51 & 68.33 & 62.78 \\
            & SmoothQuant & 163.6\ts{*} & 54.70 & 55.40 & 51.50 & 43.90 & 27.70 & 38.90 & 45.35 \\
            & LLM-QAT & 11.6\ts{*} & 69.50 & 75.40 & 64.60 & 66.00 & \u{43.80} & 69.20 & 64.75 \\
            % & (QoQ) & (5.93) & - & - & - & - & - & - & - \\
            & PEQA (our impl.) & 6.15 & 72.97 & 77.80 & \u{67.72} & 67.13 & 40.27 & \u{73.35} & 66.54 \\
            & \gcb{LR-QAT (ours)} & \gcb{6.07} & \gcb{73.64} & \gcb{77.91} & \gc{67.56} & \gcb{69.28} & \gc{41.30} & \gc{73.25} & \gcb{67.16} \\
            \midrule
            %
            %
            \multirow{7}{*}{\shortstack{4-4-4}} 
            & RTN & 17.75 & 50.49 & 64.25 & 52.41 & 48.27 & 30.12 & 52.04 & 49.60 \\
            & SmoothQuant & 25.25 & 49.10 & 49.80 & 48.00 & 30.40 & 25.80 & 27.40 & 38.42 \\
            & LLM-QAT & - & 61.30 & 51.50 & 51.90 & 27.90 & 23.90 & 31.10 & 41.27 \\
            & LLM-QAT + SQ & - & 62.40 & 55.90 & 50.60 & 35.50 & 26.40 & 47.80 & 46.43 \\
            & OS+ & - & 60.21 & 62.73 & 52.96 & 39.98 & 30.29 & 44.39 & 48.43 \\
            & OmniQuant\ts{\S} & 11.26 & 63.51 & 66.15 & 53.43 & 45.20 & 31.14 & 56.44 & 52.65 \\
            & PEQA (our impl.) & 8.60 & 65.69 & \u{72.31} & \u{59.83} & 56.52 & 34.22 & 61.79 & 58.39 \\
            & \gcb{LR-QAT (ours)} & \gcb{8.47} & \gcb{67.16} & \gc{71.76} & \gc{59.59} & \gcb{58.42} & \gcb{34.73} & \gcb{62.34} & \gcb{59.00} \\
            %
            %
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


==> tables/_archive/A_2_bit_zero_shot.tex <==
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval 2-bit (asymmetric) weight quantization results for {\llama}-2 7B}. 
    We report zero-shot accuracy of 6 tasks (higher is better).}
    \label{tbl:A_2_bit_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{clccccccc}
            \toprule
            {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            \midrule
            % \cmidrule[0.5pt]{1-10}
            %
            %
            \multirow{3}{*}{W2\,pc} & RTN & 39.57 & 50.71 & 50.20 & 26.73 & 26.28 & 25.63 & 36.52 \\
            & PEQA (our impl.) & 64.98 & 71.33 & 58.09 & 55.22 & 33.11 & 61.66 & 57.40 \\            
            & \gcb{LR-QAT (ours)} & \gcb{69.88} & \gcb{73.07} & \gcb{62.90} & \gcb{56.57} & \gcb{34.04} & \gcb{63.71} & \gcb{60.03} \\
            %
            \midrule
            % 
            \multirow{3}{*}{W2\,g128} & RTN & 39.08 & 55.93 & 50.99 & 29.84 & 24.06 & 27.71 & 37.94 \\
            & PEQA (our impl.) & 69.51 & 73.83 & 63.46 & 58.21 & 34.90 & 64.53 & 60.74 \\
            & \gcb{LR-QAT (ours)} & \gcb{70.18} & \gcb{73.83} & \gcb{63.69} & \gcb{60.27} & \gcb{34.98} & \gcb{67.24} & \gcb{61.70} \\
            % 
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}



==> tables/_archive/A_rtn.old.tex <==
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{A comparison between min-max and the best range setting used for round-to-nearest (RTN) initialization for {\llama} and Mistral models}. 
    We report WikiText-2 test set perplexity (lower is better) and average zero-shot accuracy (higher is better). Numbers marked in bold are the best results.}
    \label{tbl:A_rtn}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{0.8\columnwidth}{!}{%
        \begin{tabular}{lclcc}
            \toprule
            % \cmidrule[1]{1-5}
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{RTN init.} & WikiText-2 $\da$ & Zero-shot accuracy $\ua$ \\
            % \midrule
            % \specialrule{0.75pt}{1pt}{1pt}
            \cmidrule[0.5pt]{1-5}
            %
            % 
            \multirow{9}{*}{\shortstack{{\llama}-1 7B}}
            & FP16 &  & 5.68 & 69.68 \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,pc}} & min-max & 6.85 & 66.23 \\
            & & \gcb{best ($L^4$)} & \gcb{6.33} & \gcb{68.51} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,pc}} & min-max & 2.4e4 & 36.02 \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{12.88} & \gcb{54.66} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,g128}} & min-max & 6.08 & \u{68.96} \\
            & & \gcb{best ($L^5$)} & \gcb{6.05} & \gc{68.93} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,g128}} & min-max & 8.10 & 62.69 \\
            & & \gcb{best ($L^5$)} & \gcb{7.95} & \gcb{63.50} \\
            % 
            % 
            \cmidrule[0.5pt]{1-5}
            \multirow{8}{*}{\shortstack{{\llama}-2 7B}}
            % 
            & FP16 &  & 5.47 & 70.47 \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,pc}} & min-max & 7.14 & 66.41 \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{6.14} & \gcb{68.88} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,pc}} & min-max & 1.9e4 & 35.71 \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{26.73} & \gcb{43.87} \\
            \cmidrule{2-5}
            & \multirow{1}{*}{\shortstack{W4\,g128}} & \u{best = min-max} & \u{5.78} & \u{69.75} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,g128}} & min-max & 8.22 & \u{64.07} \\
            & & \gcb{best ($L^4$)} & \gcb{7.61} & \gc{63.20} \\
            %
            %
            % \midrule
            \cmidrule[0.5pt]{1-5}
            \multirow{8}{*}{\shortstack{{\llama}-2 13B}}
            & FP16 &  & 4.88 & 73.18 \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,pc}} & min-max & 5.40 & \u{72.19} \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{5.21} & \gc{71.73} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,pc}} & min-max & 2.3e3 & 37.85 \\
            & & \gcb{best ($L^5$)} & \gcb{8.71} & \gcb{55.01} \\
            \cmidrule{2-5}
            & \multirow{1}{*}{\shortstack{W4\,g128}} & \u{best = min-max} & \u{5.04} & \u{72.94} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,g128}} & min-max & \u{6.14} & 66.81 \\
            & & \gcb{best ($L^5$)} & \gc{6.20} & \gcb{67.60} \\
            % 
            % 
            % \midrule
            \cmidrule[0.5pt]{1-5}
            \multirow{9}{*}{\shortstack{{\llama}-3 8B}}
            & FP16 &  & 6.14 & 74.22 \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,pc}} & min-max & 10.53 & 67.44 \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{7.53} & \gcb{72.19} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,pc}} & min-max & 1.6e5 & 35.78 \\
            & & \gcb{best ($L^{3.5}$)} & \gcb{34.10} & \gcb{47.46} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,g128}} & min-max & 6.99 & \u{72.95} \\
            & & \gcb{best ($L^4$)} & \gcb{6.96} & \gc{72.30} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,g128}} & min-max & 29.38 & 54.54 \\
            & & \gcb{best ($L^5$)} & \gcb{15.11} & \gcb{57.74} \\
            %
            %
            % \midrule
            \cmidrule[0.5pt]{1-5}
            \multirow{9}{*}{\shortstack{Mistral 7B}}
            & FP16 &  & 5.25 & 75.69 \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,pc}} & min-max & 6.33 & 71.84 \\
            & & \gcb{best ($L^4$)} & \gcb{5.91} & \gcb{73.44} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,pc}} & min-max & 3.2e3 & 36.78 \\
            & & \gcb{best ($L^4$)} & \gcb{9.49} & \gcb{64.58} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W4\,g128}} & min-max & 5.51 & 74.98 \\
            & & \gcb{best ($L^5$)} & \gcb{5.49} & \gcb{75.07} \\
            \cmidrule{2-5}
            & \multirow{2}{*}{\shortstack{W3\,g128}} & min-max & 7.22 & 68.35 \\
            & & \gcb{best ($L^5$)} & \gcb{6.77} & \gcb{69.35} \\
            % 
            % 
            \bottomrule
            % \cmidrule[1.0]{1-5}
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


==> tables/_archive/A_weights_only_zero_shot.tex <==
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for {\llama} and Mistral models}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. }
    \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % \midrule
            \cmidrule[0.5pt]{1-10}
            %
            % 
            % 
            \multirow{15}{*}{{{\llama}-1 7B}}
            % 
            & FP16 &  & 75.05 & 79.16 & 70.01 & 72.85 & 44.80 & 76.21 & 69.68 \\
            \cmidrule{2-10}
            & \multirow{5}{*}{W4\,pc} & RTN & 73.18 & 78.78 & 69.14 & 71.38 & 44.37 & 74.22 & 68.51 \\
            & & GPTQ\ts{\S} & 67.70 & 76.00 & 66.70 & 66.90 & 43.00 & 69.40 & 64.95 \\
            & & LLM-QAT & {75.50} & {78.30} & 69.00 & 70.00 & {45.00} & 74.00 & {68.63} \\
            & & PEQA (our impl.) & 74.71 & 78.29 & 70.09 & 70.33 & 42.24 & 75.27 & 68.49 \\
            & & \gcb{LR-QAT (ours)} & \gcb{74.13} & \gcb{78.29} & \gcb{70.01} & \gcb{71.21} & \gcb{42.41} & \gcb{75.16} & \gcb{68.54} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{W3\,pc} & RTN & 58.93 & 70.40 & 55.72 & 55.01 & 32.17 & 55.75 & 54.66 \\
            & & PEQA (our impl.) & 72.69 & 77.15 & 65.90 & 68.27 & 38.91 & 71.60 & 65.75 \\
            & & \gcb{LR-QAT (ours)} & \gcb{73.24} & \gcb{78.18} & \gcb{67.40} & \gcb{67.47} & \gcb{40.53} & \gcb{72.77} & \gcb{66.60} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{W4\,g128} & RTN & 74.77 & 78.51 & {70.64} & 71.30 & 43.60 & 74.74 & 68.93 \\
            & & PEQA (our impl.) & 75.75 & 79.17 & 70.17 & 70.75 & 43.60 & 75.71 & 69.19 \\
            & & \gcb{LR-QAT (ours)} & \gcb{75.29} & \gcb{78.62} & \gcb{69.61} & \gcb{71.59} & \gcb{44.11} & \gcb{75.67} & \gcb{69.15} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{W3\,g128} & RTN & 69.48 & 76.33 & 64.40 & 64.44 & 38.65 & 67.67 & 63.50 \\
            & & PEQA (our impl.) & 71.65 & 78.24 & 68.51 & 68.18 & 40.10 & 73.30 & 66.66 \\
            & & \gcb{LR-QAT (ours)} & \gcb{72.84} & \gcb{78.02} & \gcb{67.40} & \gcb{68.52} & \gcb{41.04} & \gcb{73.04} & \gcb{66.81} \\
            % 
            \midrule
            % 
            % 
            % 
            \multirow{13}{*}{{{\llama}-2 7B}}
            % 
            & FP16 &  & 77.74 & 79.11 & 69.14 & 74.58 & 46.25 & 75.98 & 70.47 \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,pc}} & RTN & 76.36 & 78.07 & 68.19 & 71.21 & 44.80 & 74.65 & 68.88 \\
            & & PEQA (our impl.) & 77.49 & 78.24 & 69.61 & 70.96 & 43.52 & 75.54 & 69.23 \\
            & & \gcb{LR-QAT (ours)} & \gcb{77.43} & \gcb{78.45} & \gcb{69.69} & \gcb{73.15} & \gcb{45.48} & \gcb{75.51} & \gcb{69.95} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,pc}} & RTN & 46.27 & 60.28 & 54.85 & 38.05 & 23.29 & 40.47 & 43.87 \\
            & & PEQA (our impl.) & 71.62 & 76.82 & 66.14 & 65.66 & 39.76 & 72.63 & 65.44 \\
            & & \gcb{LR-QAT (ours)} & \gcb{74.43} & \gcb{77.15} & \gcb{68.03} & \gcb{69.95} & \gcb{43.09} & \gcb{73.29} & \gcb{67.66} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,g128}} & RTN & 76.76 & 78.18 & 69.77 & 72.60 & 45.73 & 75.43 & 69.75 \\
            & & PEQA (our impl.) & 76.88 & 78.89 & 69.85 & 72.18 & 44.11 & 75.95 & 69.64 \\
            & & \gcb{LR-QAT (ours)} & \gcb{76.73} & \gcb{78.62} & \gcb{70.48} & \gcb{72.85} & \gcb{44.97} & \gcb{75.62} & \gcb{69.88} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,g128}} & RTN & 66.42 & 75.57 & 65.19 & 64.90 & 38.14 & 68.96 & 63.20 \\
            & & PEQA (our impl.) & 75.38 & 77.97 & 68.59 & 70.62 & 42.32 & 73.74 & 68.10 \\
            & & \gcb{LR-QAT (ours)} & \gcb{76.61} & \gcb{77.31} & \gcb{68.98} & \gcb{72.05} & \gcb{42.58} & \gcb{74.20} & \gcb{68.62} \\
            % 
            % 
            % \midrule
            \cmidrule[0.5pt]{1-10}
            \multirow{13}{*}{{{\llama}-2 13B}}
            % 
            & FP16 &  & 80.55 & 80.52 & 72.22 & 77.44 & 48.98 & 79.38 & 73.18 \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,pc}} & RTN & 79.30 & 79.71 & 70.01 & 75.51 & 48.89 & 76.96 & 71.73 \\
            & & PEQA (our impl.) & 78.99 & 80.14 & 71.27 & 76.43 & 48.98 & 79.24 & 72.51 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.15} & \gcb{80.09} & \gcb{72.06} & \gcb{77.65} & \gcb{49.91} & \gcb{79.28} & \gcb{73.19} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,pc}} & RTN & 55.05 & 71.06 & 54.22 & 56.19 & 32.25 & 61.27 & 55.01 \\
            & & PEQA (our impl.) & 74.28 & 78.67 & 69.06 & 74.87 & 45.99 & 76.00 & 69.81 \\
            & & \gcb{LR-QAT (ours)} & \gcb{78.62} & \gcb{79.49} & \gcb{72.61} & \gcb{73.99} & \gcb{45.56} & \gcb{77.05} & \gcb{71.22} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,g128}} & RTN & 81.10 & 79.82 & 72.38 & 76.73 & 49.06 & 78.52 & 72.94 \\
            & & PEQA (our impl.) & 80.28 & 80.63 & 71.74 & 76.14 & 48.38 & 79.62 & 72.80 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.73} & \gcb{80.30} & \gcb{71.74} & \gcb{76.14} & \gcb{49.06} & \gcb{79.51} & \gcb{72.91} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,g128}} & RTN & 74.65 & 76.93 & 69.14 & 70.16 & 42.66 & 72.06 & 67.60 \\
            & & PEQA (our impl.) & 78.56 & 78.73 & 69.85 & 73.61 & 44.28 & 76.69 & 70.29 \\
            & & \gcb{LR-QAT (ours)} & \gcb{79.79} & \gcb{79.60} & \gcb{70.64} & \gcb{74.24} & \gcb{46.76} & \gcb{78.00} & \gcb{71.51} \\
            % 
            % 
            % \midrule
            \cmidrule[0.5pt]{1-10}
            \multirow{13}{*}{{{\llama}-3 8B}}
            % 
            & FP16 &  & 81.44 & 80.79 & 72.85 & 77.74 & 53.33 & 79.16 & 74.22 \\
            % 
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,pc}} & RTN & 79.02 & 78.56 & 72.85 & 75.97 & 49.32 & 77.44 & 72.19 \\
            & & PEQA (our impl.) & 79.57 & 78.67 & 72.93 & 77.19 & 51.11 & 77.25 & 72.79 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.62} & \gcb{79.98} & \gcb{72.85} & \gcb{78.32} & \gcb{52.05} & \gcb{78.19} & \gcb{73.84} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,pc}} & RTN & 58.65 & 61.75 & 56.04 & 39.60 & 23.81 & 44.91 & 47.46 \\
            & & PEQA (our impl.) & 63.18 & 64.74 & 57.62 & 43.39 & 26.88 & 50.48 & 51.05 \\
            & & \gcb{LR-QAT (ours)} & \gcb{77.46} & \gcb{78.51} & \gcb{69.85} & \gcb{74.83} & \gcb{47.35} & \gcb{74.73} & \gcb{70.46} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,g128}} & RTN & 79.48 & 79.27 & 73.56 & 75.08 & 48.81 & 77.61 & 72.30 \\
            & & PEQA (our impl.) & 80.98 & 80.14 & 72.61 & 76.18 & 49.57 & 78.45 & 72.99 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.40} & \gcb{80.90} & \gcb{73.48} & \gcb{77.44} & \gcb{51.11} & \gcb{78.60} & \gcb{73.66} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,g128}} & RTN & 65.47 & 68.39 & 65.19 & 54.00 & 33.45 & 59.96 & 57.74 \\
            & & PEQA (our impl.) & 72.26 & 76.06 & 67.80 & 69.02 & 46.08 & 71.89 & 67.19 \\
            & & \gcb{LR-QAT (ours)} & \gcb{72.97} & \gcb{79.38} & \gcb{71.67} & \gcb{74.37} & \gcb{49.06} & \gcb{75.44} & \gcb{70.48} \\
            % 
            %
            % \midrule
            \cmidrule[0.5pt]{1-10}
            \multirow{13}{*}{{Mistral 7B}}
            % 
            & FP16 &  & 83.58 & 82.10 & 73.88 & 79.59 & 53.92 & 81.07 & 75.69 \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,pc}} & RTN & 81.22 & 80.63 & 72.53 & 76.77 & 50.09 & 79.41 & 73.44 \\
            & & PEQA (our impl.) & 81.80 & 81.12 & 72.61 & 77.23 & 50.17 & 79.43 & 73.73 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.99} & \gcb{81.28} & \gcb{73.56} & \gcb{78.20} & \gcb{51.02} & \gcb{80.57} & \gcb{74.44} \\
            % 
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,pc}} & RTN & 68.13 & 77.64 & 63.93 & 63.93 & 41.13 & 72.73 & 64.58 \\
            & & PEQA (our impl.) & 80.03 & 80.09 & 69.93 & 72.90 & 45.82 & 77.32 & 71.02 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.62} & \gcb{80.09} & \gcb{70.96} & \gcb{74.75} & \gcb{46.08} & \gcb{77.71} & \gcb{71.87} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W4\,g128}} & RTN & 84.16 & 81.77 & 74.43 & 77.95 & 51.71 & 80.42 & 75.07 \\
            & & PEQA (our impl.) & 80.89 & 81.72 & 73.80 & 75.42 & 48.46 & 79.76 & 73.34 \\
            & & \gcb{LR-QAT (ours)} & \gcb{83.55} & \gcb{81.61} & \gcb{74.51} & \gcb{78.28} & \gcb{52.90} & \gcb{80.84} & \gcb{75.28} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{{W3\,g128}} & RTN & 78.44 & 79.60 & 69.14 & 71.17 & 43.00 & 74.75 & 69.35 \\
            & & PEQA (our impl.) & 81.99 & 81.18 & 69.61 & 74.92 & 47.18 & 78.37 & 72.21 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.71} & \gcb{80.90} & \gcb{70.48} & \gcb{75.08} & \gcb{47.78} & \gcb{78.50} & \gcb{72.41} \\
            %
            %
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


==> tables/_archive/A_weights_only_zero_shot_v2.tex <==
% 
% #
% ##
% ### L1-7B
% 
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for {\llama}-1 7B}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. }
    % \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % \midrule
            \cmidrule[0.5pt]{1-10}
            %
            % 
            % 
            \multirow{25}{*}{{{\llama}-1 7B}}
            % 
            & FP16 &  & 75.05 & 79.16 & 70.01 & 72.85 & 44.80 & 76.21 & 69.68 \\
            \cmidrule{2-10}
            & \multirow{6}{*}{\shortstack{W4\,pc}} & RTN & 73.18 & 78.78 & 69.14 & 71.38 & 44.37 & 74.22 & 68.51 \\
            & & GPTQ\ts{\S} & 67.70 & 76.00 & 66.70 & 66.90 & 43.00 & 69.40 & 64.95 \\
            & & LLM-QAT & 75.50 & 78.30 & 69.00 & 70.00 & 45.00 & 74.00 & 68.63 \\
            & & LSQ (our impl.) & 73.91 & 78.24 & 69.22 & 70.84 & 43.26 & 74.74 & 68.37 \\
            & & PEQA (our impl.) & 74.71 & 78.29 & 70.09 & 70.33 & 42.24 & 75.27 & 68.49 \\
            & & \gcb{LR-QAT (ours)} & \gcb{74.13} & \gcb{78.29} & \gcb{70.01} & \gcb{71.21} & \gcb{42.41} & \gcb{75.16} & \gcb{68.54} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,g128}} & RTN & 74.77 & 78.51 & 70.64 & 71.30 & 43.60 & 74.74 & 68.93 \\
            & & LSQ (our impl.) & 75.90 & 79.22 & 70.01 & 71.42 & 43.34 & 75.15 & 69.17 \\
            & & PEQA (our impl.) & 75.75 & 79.17 & 70.17 & 70.75 & 43.60 & 75.71 & 69.19 \\
            & & \gcb{LR-QAT (ours)} & \gcb{75.29} & \gcb{78.62} & \gcb{69.61} & \gcb{71.59} & \gcb{44.11} & \gcb{75.67} & \gcb{69.15} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,pc}} & RTN & 58.93 & 70.40 & 55.72 & 55.01 & 32.17 & 55.75 & 54.66 \\
            & & LSQ (our impl.) & 71.35 & 77.97 & 68.82 & 66.33 & 40.10 & 73.14 & 66.29 \\
            & & PEQA (our impl.) & 72.69 & 77.15 & 65.90 & 68.27 & 38.91 & 71.60 & 65.75 \\
            & & \gcb{LR-QAT (ours)} & \gcb{73.24} & \gcb{78.18} & \gcb{67.40} & \gcb{67.47} & \gcb{40.53} & \gcb{72.77} & \gcb{66.60} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,g128}} & RTN & 69.48 & 76.33 & 64.40 & 64.44 & 38.65 & 67.67 & 63.50 \\
            & & LSQ (our impl.) & 71.04 & 77.97 & 68.11 & 68.27 & 40.44 & 73.37 & 66.53 \\
            & & PEQA (our impl.) & 71.65 & 78.24 & 68.51 & 68.18 & 40.10 & 73.30 & 66.66 \\
            & & \gcb{LR-QAT (ours)} & \gcb{72.84} & \gcb{78.02} & \gcb{67.40} & \gcb{68.52} & \gcb{41.04} & \gcb{73.04} & \gcb{66.81} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,pc}} & RTN\ts{\S} & 43.24 & 52.61 & 51.62 & 27.48 & 26.28 & 26.26 & 37.92 \\
            & & PEQA (our impl.)\ts{\S} & 67.19 & 74.32 & 61.80 & 59.97 & 32.42 & 63.28 & 59.83 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{68.07} & \gcb{74.27} & \gcb{64.80} & \gcb{61.03} & \gcb{36.95} & \gcb{65.48} & \gcb{61.77} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,g128}} & RTN\ts{\S} & 41.16 & 58.05 & 50.20 & 34.97 & 23.12 & 30.93 & 39.74 \\
            & & PEQA (our impl.)\ts{\S} & 67.40 & 74.21 & 62.04 & 60.98 & 35.32 & 64.16 & 60.69 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{67.65} & \gcb{74.86} & \gcb{61.80} & \gcb{62.37} & \gcb{37.03} & \gcb{65.90} & \gcb{61.60} \\
            %
            %
            %
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


% 
% #
% ##
% ### L2-7B
% 
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for {\llama}-2 7B}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. }
    % \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % \midrule
            \cmidrule[0.5pt]{1-10}
            \multirow{23}{*}{{{\llama}-2 7B}}
            % 
            & FP16 &  & 77.74 & 79.11 & 69.14 & 74.58 & 46.25 & 75.98 & 70.47 \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,pc}} & RTN & 76.36 & 78.07 & 68.19 & 71.21 & 44.80 & 74.65 & 68.88 \\
            & & LSQ (our impl.) & 76.69 & 78.15 & 68.12 & 71.84 & 44.18 & 74.76 & 68.96 \\
            & & PEQA (our impl.) & 77.49 & 78.24 & 69.61 & 70.96 & 43.52 & 75.54 & 69.23 \\
            & & \gcb{LR-QAT (ours)} & \gcb{77.41} & \gcb{78.56} & \gcb{69.42} & \gcb{72.80} & \gcb{44.66} & \gcb{75.45} & \gcb{69.72} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,g128}} & RTN & 76.76 & 78.18 & 69.77 & 72.60 & 45.73 & 75.43 & 69.75 \\
            & & LSQ (our impl.) & 77.28 & 78.45 & 69.61 & 72.18 & 44.97 & 75.61 & 69.68 \\
            & & PEQA (our impl.) & 76.88 & 78.89 & 69.85 & 72.18 & 44.11 & 75.95 & 69.64 \\
            & & \gcb{LR-QAT (ours)} & \gcb{76.73} & \gcb{78.62} & \gcb{70.48} & \gcb{72.85} & \gcb{44.97} & \gcb{75.62} & \gcb{69.88} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,pc}} & RTN & 46.27 & 60.28 & 54.85 & 38.05 & 23.29 & 40.47 & 43.87 \\
            & & LSQ (our impl.) & 74.39 & 77.91 & 66.85 & 69.15 & 41.53 & 73.04 & 67.14 \\
            & & PEQA (our impl.) & 71.62 & 76.82 & 66.14 & 65.66 & 39.76 & 72.63 & 65.44 \\
            & & \gcb{LR-QAT (ours)} & \gcb{75.08} & \gcb{77.73} & \gcb{67.50} & \gcb{69.97} & \gcb{42.70} & \gcb{73.24} & \gcb{67.70} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,g128}} & RTN & 66.42 & 75.57 & 65.19 & 64.90 & 38.14 & 68.96 & 63.20 \\
            & & LSQ (our impl.) & 74.68 & 77.80 & 68.35 & 71.76 & 44.11 & 73.46 & 68.36 \\
            & & PEQA (our impl.) & 75.38 & 77.97 & 68.59 & 70.62 & 42.32 & 73.74 & 68.10 \\
            & & \gcb{LR-QAT (ours)} & \gcb{76.61} & \gcb{77.31} & \gcb{68.98} & \gcb{72.05} & \gcb{42.58} & \gcb{74.20} & \gcb{68.62} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,pc}} & RTN\ts{\S} & 39.57 & 50.71 & 50.20 & 26.73 & 26.28 & 25.63 & 36.52 \\
            & & PEQA (our impl.)\ts{\S} & 64.98 & 71.33 & 58.09 & 55.22 & 33.11 & 61.66 & 57.40 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{69.88} & \gcb{73.07} & \gcb{62.90} & \gcb{56.57} & \gcb{34.04} & \gcb{63.71} & \gcb{60.03} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,g128}} & RTN\ts{\S} & 39.08 & 55.93 & 50.99 & 29.84 & 24.06 & 27.71 & 37.94 \\
            & & PEQA (our impl.)\ts{\S} & 69.51 & 73.83 & 63.46 & 58.21 & 34.90 & 64.53 & 60.74 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{70.18} & \gcb{73.83} & \gcb{63.69} & \gcb{60.27} & \gcb{34.98} & \gcb{67.24} & \gcb{61.70} \\
            % 
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


% 
% #
% ##
% ### L2-13B
% 
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for {\llama}-2 13B}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. {\oom} denotes out of memory.}
    % \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % 
            \cmidrule[0.5pt]{1-10}
            \multirow{23}{*}{{{\llama}-2 13B}}
            % 
            & FP16 &  & 80.55 & 80.52 & 72.22 & 77.44 & 48.98 & 79.38 & 73.18 \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,pc}} & RTN & 79.30 & 79.71 & 70.01 & 75.51 & 48.89 & 76.96 & 71.73 \\
            & & LSQ (our impl.) & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} \\
            & & PEQA (our impl.) & 78.99 & 80.14 & 71.27 & 76.43 & 48.98 & 79.24 & 72.51 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.15} & \gcb{80.09} & \gcb{72.06} & \gcb{77.65} & \gcb{49.91} & \gcb{79.28} & \gcb{73.19} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,g128}} & RTN & 81.10 & 79.82 & 72.38 & 76.73 & 49.06 & 78.52 & 72.94 \\
            & & LSQ (our impl.) & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} \\
            & & PEQA (our impl.) & 80.28 & 80.63 & 71.74 & 76.14 & 48.38 & 79.62 & 72.80 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.73} & \gcb{80.30} & \gcb{71.74} & \gcb{76.14} & \gcb{49.06} & \gcb{79.51} & \gcb{72.91} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,pc}} & RTN & 55.05 & 71.06 & 54.22 & 56.19 & 32.25 & 61.27 & 55.01 \\
            & & LSQ (our impl.) & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} \\
            & & PEQA (our impl.) & 74.28 & 78.67 & 69.06 & 74.87 & 45.99 & 76.00 & 69.81 \\
            & & \gcb{LR-QAT (ours)} & \gcb{78.62} & \gcb{79.49} & \gcb{72.61} & \gcb{73.99} & \gcb{45.56} & \gcb{77.05} & \gcb{71.22} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,g128}} & RTN & 74.65 & 76.93 & 69.14 & 70.16 & 42.66 & 72.06 & 67.60 \\
            & & LSQ (our impl.) & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} & {\oom} \\
            & & PEQA (our impl.) & 78.56 & 78.73 & 69.85 & 73.61 & 44.28 & 76.69 & 70.29 \\
            & & \gcb{LR-QAT (ours)} & \gcb{79.79} & \gcb{79.60} & \gcb{70.64} & \gcb{74.24} & \gcb{46.76} & \gcb{78.00} & \gcb{71.51} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,pc}} & RTN\ts{\S} & 38.35 & 48.97 & 48.54 & 27.78 & 27.99 & 25.97 & 36.27 \\
            & & PEQA (our impl.)\ts{\S} & 71.19 & 74.48 & 59.67 & 62.96 & 37.29 & 68.14 & 62.29 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{72.60} & \gcb{76.61} & \gcb{66.22} & \gcb{66.67} & \gcb{39.76} & \gcb{69.79} & \gcb{65.28} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,g128}} & RTN\ts{\S} & 50.12 & 57.29 & 50.36 & 34.43 & 22.18 & 32.35 & 41.12 \\
            & & PEQA (our impl.)\ts{\S} & 70.34 & 76.88 & 66.85 & 64.94 & 38.74 & 70.66 & 64.74 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{75.47} & \gcb{77.86} & \gcb{65.98} & \gcb{67.63} & \gcb{41.04} & \gcb{72.50} & \gcb{66.75} \\
            % 
            % 
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


% 
% #
% ##
% ### L3-8B
% 
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for {\llama}-3 8B}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. }
    \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % 
            % 
            % \midrule
            \cmidrule[0.5pt]{1-10}
            \multirow{23}{*}{{{\llama}-3 8B}}
            % 
            & FP16 &  & 81.44 & 80.79 & 72.85 & 77.74 & 53.33 & 79.16 & 74.22 \\
            % 
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,pc}} & RTN & 79.02 & 78.56 & 72.85 & 75.97 & 49.32 & 77.44 & 72.19 \\
            & & LSQ (our impl.) & 80.58 & 80.03 & 72.69 & 78.24 & 50.17 & 77.94 & 73.28 \\
            & & PEQA (our impl.) & 79.57 & 78.67 & 72.93 & 77.19 & 51.11 & 77.25 & 72.79 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.62} & \gcb{79.98} & \gcb{72.85} & \gcb{78.32} & \gcb{52.05} & \gcb{78.19} & \gcb{73.84} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,g128}} & RTN & 79.48 & 79.27 & 73.56 & 75.08 & 48.81 & 77.61 & 72.30 \\
            & & LSQ (our impl.) & 80.24 & 80.36 & 73.01 & 77.23 & 50.43 & 78.60 & 73.31 \\
            & & PEQA (our impl.) & 80.98 & 80.14 & 72.61 & 76.18 & 49.57 & 78.45 & 72.99 \\
            & & \gcb{LR-QAT (ours)} & \gcb{80.40} & \gcb{80.90} & \gcb{73.48} & \gcb{77.44} & \gcb{51.11} & \gcb{78.60} & \gcb{73.66} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,pc}} & RTN & 58.65 & 61.75 & 56.04 & 39.60 & 23.81 & 44.91 & 47.46 \\
            & & LSQ (our impl.) & 76.42 & 78.24 & 70.01 & 72.31 & 45.22 & 75.26 & 69.58 \\
            & & PEQA (our impl.) & 63.18 & 64.74 & 57.62 & 43.39 & 26.88 & 50.48 & 51.05 \\
            & & \gcb{LR-QAT (ours)} & \gcb{77.46} & \gcb{78.51} & \gcb{69.85} & \gcb{74.83} & \gcb{47.35} & \gcb{74.73} & \gcb{70.46} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,g128}} & RTN & 65.47 & 68.39 & 65.19 & 54.00 & 33.45 & 59.96 & 57.74 \\
            & & LSQ (our impl.) & 75.50 & 78.78 & 69.69 & 73.57 & 48.55 & 74.55 & 70.11 \\
            & & PEQA (our impl.) & 72.26 & 76.06 & 67.80 & 69.02 & 46.08 & 71.89 & 67.19 \\
            & & \gcb{LR-QAT (ours)} & \gcb{72.97} & \gcb{79.38} & \gcb{71.67} & \gcb{74.37} & \gcb{49.06} & \gcb{75.44} & \gcb{70.48} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,pc}} & RTN\ts{\S} & 44.89 & 48.97 & 47.51 & 25.29 & 27.73 & 26.41 & 36.80 \\
            & & PEQA (our impl.)\ts{\S} & 62.54 & 72.96 & 59.51 & 56.82 & 33.70 & 60.77 & 57.72 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{65.81} & \gcb{72.31} & \gcb{64.72} & \gcb{53.54} & \gcb{33.45} & \gcb{61.11} & \gcb{58.49} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,g128}} & RTN\ts{\S} & 38.47 & 53.32 & 51.78 & 28.75 & 22.70 & 26.81 & 36.97 \\
            & & PEQA (our impl.)\ts{\S} & 58.53 & 72.52 & 61.96 & 57.41 & 35.32 & 61.14 & 57.81 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{67.98} & \gcb{73.83} & \gcb{62.83} & \gcb{56.94} & \gcb{36.43} & \gcb{64.77} & \gcb{60.46} \\
            %
            %
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


% 
% #
% ##
% ### M-7B
% 
\begin{table*}[htb]
    \setlength{\tabcolsep}{6pt}
    % \small
    \centering
    \caption{\textbf{LM-eval weight-only quantization results for Mistral 7B}. We report zero-shot accuracy of 6 tasks (higher is better). {\ts{\S}}Uses asymmetric weight quantization. }
    % \label{tbl:A_weight_only_zero_shot}
    \renewcommand{\arraystretch}{0.9}
    % 
    \resizebox{1\columnwidth}{!}{%
        \begin{tabular}{lclccccccc}
            \toprule
            \multicolumn{1}{c}{Model} & {\# Bits} & \multicolumn{1}{c}{Method} & BoolQ & PIQA & Winogrande & ARC-e & ARC-c & HellaSwag & {Avg.} \\
            % \midrule
            % 
            % 
            \cmidrule[0.5pt]{1-10}
            \multirow{23}{*}{{Mistral 7B}}
            % 
            & FP16 &  & 83.58 & 82.10 & 73.88 & 79.59 & 53.92 & 81.07 & 75.69 \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,pc}} & RTN & 81.22 & 80.63 & 72.53 & 76.77 & 50.09 & 79.41 & 73.44 \\
            & & LSQ (our impl.) & 81.96 & 80.41 & 73.09 & 75.08 & 48.55 & 78.19 & 72.88 \\
            & & PEQA (our impl.) & 81.80 & 81.12 & 72.61 & 77.23 & 50.17 & 79.43 & 73.73 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.99} & \gcb{81.28} & \gcb{73.56} & \gcb{78.20} & \gcb{51.02} & \gcb{80.57} & \gcb{74.44} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W4\,g128}} & RTN & 84.16 & 81.77 & 74.43 & 77.95 & 51.71 & 80.42 & 75.07 \\
            & & LSQ (our impl.) & 80.40 & 80.63 & 73.16 & 76.26 & 48.72 & 78.24 & 72.90 \\
            & & PEQA (our impl.) & 80.89 & 81.72 & 73.80 & 75.42 & 48.46 & 79.76 & 73.34 \\
            & & \gcb{LR-QAT (ours)} & \gcb{83.55} & \gcb{81.61} & \gcb{74.51} & \gcb{78.28} & \gcb{52.90} & \gcb{80.84} & \gcb{75.28} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,pc}} & RTN & 68.13 & 77.64 & 63.93 & 63.93 & 41.13 & 72.73 & 64.58 \\
            & & LSQ (our impl.) & 79.97 & 80.74 & 70.24 & 74.37 & 47.18 & 77.14 & 71.61 \\
            & & PEQA (our impl.) & 80.03 & 80.09 & 69.93 & 72.90 & 45.82 & 77.32 & 71.02 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.62} & \gcb{80.09} & \gcb{70.96} & \gcb{74.75} & \gcb{46.08} & \gcb{77.71} & \gcb{71.87} \\
            \cmidrule{2-10}
            & \multirow{4}{*}{\shortstack{W3\,g128}} & RTN & 78.44 & 79.60 & 69.14 & 71.17 & 43.00 & 74.75 & 69.35 \\
            & & LSQ (our impl.) & 81.01 & 80.36 & 71.03 & 74.41 & 47.27 & 77.68 & 71.96 \\
            & & PEQA (our impl.) & 81.99 & 81.18 & 69.61 & 74.92 & 47.18 & 78.37 & 72.21 \\
            & & \gcb{LR-QAT (ours)} & \gcb{81.71} & \gcb{80.90} & \gcb{70.48} & \gcb{75.08} & \gcb{47.78} & \gcb{78.50} & \gcb{72.41} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,pc}} & RTN\ts{\S} & 39.42 & 51.03 & 49.49 & 26.22 & 26.71 & 26.67 & 36.59 \\
            & & PEQA (our impl.)\ts{\S} & 74.34 & 75.95 & 66.22 & 62.21 & 38.48 & 69.68 & 64.48 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{75.08} & \gcb{76.39} & \gcb{65.98} & \gcb{64.48} & \gcb{39.59} & \gcb{69.14} & \gcb{65.11} \\
            \cmidrule{2-10}
            & \multirow{3}{*}{\shortstack{W2\,g128}} & RTN\ts{\S} & 54.98 & 56.91 & 51.70 & 31.27 & 23.21 & 29.70 & 41.30 \\
            & & PEQA (our impl.)\ts{\S} & 75.41 & 75.84 & 64.96 & 65.45 & 38.23 & 68.00 & 64.65 \\
            & & \gcb{LR-QAT (ours)\ts{\S}} & \gcb{75.81} & \gcb{77.15} & \gcb{64.64} & \gcb{63.59} & \gcb{39.51} & \gcb{70.89} & \gcb{65.27} \\
            %
            %
            \bottomrule
            % 
        \end{tabular}
    }  % end resizebox
    \vspace{-.1cm}
\end{table*}


==> tables/_archive/_04_ablation_lora_rank.tex <==
% 
%
\begin{table*}[htb]
    \centering
    \begin{tabular}{ ccc }
        \toprule
         LoRA rank, $r$ & WikiText-2 Perplexity $\da$ & Zero-shot avg. accuracy $\ua$ \\
         \midrule
         FP16 & $0$ & $0$ \\
         \midrule  
         $1$ & $0$ & $0$ \\
         $2$ & $0$ & $0$ \\
         $4$ & $0$ & $0$ \\
         $8$ & $0$ & $0$ \\
         $16$ & $0$ & $0$ \\
         $32$ & $0$ & $0$ \\
         $64$ & $0$ & $0$ \\
         $128$ & $0$ & $0$ \\
         $256$ & $0$ & $0$ \\
         \bottomrule
    \end{tabular}
    % \vspace{-.15cm}
    \caption{
    The impact of LoRa rank.
}
    \label{tbl:04_ablation_lora_rank}
\end{table*}
% 


==> tables/_archive/_mart_table.tex <==
\begin{table*}[h]
    \setlength{\tabcolsep}{6pt}
    \small
    \centering
    \caption{\textbf{Weight-only quantization results of Llama-1, Llama-2, Mistral, and Mixtral-MoE Models}. We report WikiText2 perplexity in this table; lower is better Models marked `L1' or `L2' denote Llama-v1 and Llama-v2, respectively. M denotes Mistral and 8x7B denotes Mixtral-MoE 8x7B.}
    \label{tab:extra_ppl}
    \renewcommand{\arraystretch}{0.85}
    \begin{tabular}{llccccccccc}
        \toprule
          \multicolumn{2}{l}{
          % \textbf{LLaMA1\&2; Mistral / PPL}$\downarrow$
          } & L1-7B & L1-13B & L1-30B & L1-65B & L2-7B & L2-13B & L2-70B & M-7B & 8x7B \\  \midrule
        FP16 &   & 5.68 & 5.09 & 4.10 & 3.53 & 5.47 & 4.88 & 3.31 & 5.25 & 3.84 \\ 
        \midrule
        % \multirow{3}{*}{\shortstack{W2A16}} & RTN & 1.1e5 & 6.8e4 & 2.4e4 & 2.2e4  & 3.8e4 & 5.6e4 & 2.0e4 \\
        %  & GPTQ & 2.1e3   &  5.5e3 & 499.75 & 55.91 & 7.7e3 & 2.1e3 & 77.95   \\
        %  & OmniQuant  & 15.47} & 13.21} & 8.71} &  7.58} & 37.37} & 17.21} & 7.81}   \\
        % \hline
        \multirow{6}{*}{\shortstack{2.125 bpv\\(W2@g128)}} 
         & RTN &  1.9e3  & 781.20 & 68.04 & 15.08 & 4.2e3 & 122.08 & 27.27 & 1.4e3 & 4.3e3 \\
         & GPTQ &  44.01 & 15.60 & 10.92 & 9.51 & 36.77 & 28.14 & 6.74 & 15.68 & 14.50 \\
         & AWQ &  2.6e5 & 2.8e5 & 2.4e5 & 7.4e4 & 2.2e5 & 1.2e5 & -  \\
         & OmniQuant  & 9.72 & 7.93 & 7.12 & 5.95 & 11.06 & 8.26 & 6.55  \\

         & \cellcolor{Gray}\textbf{GPTVQ 1D (ours)} 
            & \cellcolor{Gray} 16.29
            & \cellcolor{Gray} \textbf{6.93}
            & \cellcolor{Gray} \textbf{6.04}
            & \cellcolor{Gray} \textbf{5.19}
            & \cellcolor{Gray} 11.57
            & \cellcolor{Gray} \textbf{7.34}
            & \cellcolor{Gray} \textbf{5.00}
            & \cellcolor{Gray} \textbf{15.03} 
            & \cellcolor{Gray} \\
         & \cellcolor{Gray}\textbf{GPTVQ 2D (ours)} 
      & \cellcolor{Gray} \textbf{9.64}
      & \cellcolor{Gray} \textbf{6.58}
      & \cellcolor{Gray} \textbf{5.63}
      & \cellcolor{Gray} \textbf{4.91}
      & \cellcolor{Gray} \textbf{8.23}
      & \cellcolor{Gray} \textbf{6.50}
      & \cellcolor{Gray} \textbf{4.64}
      & \cellcolor{Gray} \textbf{10.28} 
            & \cellcolor{Gray}\\
         % & \cellcolor{Gray}\textbf{GPTVQ 4D (ours)} 
         %    & \cellcolor{Gray}\textbf{8.51}
         %    & \cellcolor{Gray} 
         %    & \cellcolor{Gray} 
         %    & \cellcolor{Gray} 
         %    & \cellcolor{Gray}\textbf{7.02}
         %    & \cellcolor{Gray}\textbf{5.95}
         %    & \cellcolor{Gray} 
         %    & \cellcolor{Gray}6.76\\
        \midrule
        \multirow{6}{*}{\shortstack{2.25 bpv\\(W2@g64)}} & RTN &  188.32 & 101.87 & 19.20 & 9.39  & 431.97 & 26.22 & 10.31 & 71.52 & 155.82 \\
         & GPTQ & 22.10 & 10.06 &  8.54 & 8.31 & 20.85 & 22.44 & NAN & 14.24 & 9.45 \\
         & AWQ &  2.5e5 & 2.7e5 & 2.3e5 & 7.4e4  & 2.1e5 & 1.2e5 & - \\
         & OmniQuant  & 8.90  & 7.34 & 6.59 & 5.65   & 9.62 & 7.56 & 6.11 \\ 
         & \cellcolor{Gray}\textbf{GPTVQ 1D (ours)} 
      & \cellcolor{Gray} 16.64
      & \cellcolor{Gray} \textbf{6.78}
      & \cellcolor{Gray} \textbf{5.97}
      & \cellcolor{Gray} \textbf{5.05}
      & \cellcolor{Gray} 10.08
      & \cellcolor{Gray} \textbf{7.17}
      & \cellcolor{Gray} \textbf{4.82}
      & \cellcolor{Gray} \textbf{9.56}
            & \cellcolor{Gray} \\
         & \cellcolor{Gray}\textbf{GPTVQ 2D (ours)} 
      & \cellcolor{Gray} 9.90
      & \cellcolor{Gray} \textbf{6.43}
      & \cellcolor{Gray} \textbf{5.56}
      & \cellcolor{Gray} \textbf{4.86}
      & \cellcolor{Gray} \textbf{7.97}
      & \cellcolor{Gray} \textbf{6.47}
      & \cellcolor{Gray} \textbf{4.61}
      & \cellcolor{Gray} \textbf{10.11}
            & \cellcolor{Gray} \\
        & \cellcolor{Gray}\textbf{GPTVQ 4D (ours)} 
      & \cellcolor{Gray} \textbf{8.76}
      & \cellcolor{Gray} \textbf{6.33}
      & \cellcolor{Gray} \textbf{5.42}
      & \cellcolor{Gray} \textbf{4.74}
      & \cellcolor{Gray} \textbf{7.22}
      & \cellcolor{Gray} \textbf{6.08}
      & \cellcolor{Gray} \textbf{4.39}
      & \cellcolor{Gray} \textbf{7.16}
            & \cellcolor{Gray} \\
        \midrule
        % \multirow{5}{*}{\shortstack{W3A16}} & RTN & 25.73 & 11.39 & 14.95 & 10.68 & 539.48 & 10.68 & 7.52  \\
        %  & GPTQ &  8.06 & 6.76 & 5.84 & 5.06 & 8.37 & 6.44 & 4.82 \\
        %  & AWQ & 11.88 & 7.45 & 10.07 & 5.21  & 24.00 & 10.45 & - \\
        %  & OmniQuant  & 6.49} & 5.68} & 4.74} & 4.04}  & 6.58} & 5.58} & 3.92} \\ 
        %  \hline
        \multirow{6}{*}{\shortstack{3.125 bpv\\(W3@g128)}} & RTN & 7.01 & 5.88 & 4.87 & 4.24  & 6.66 & 5.51 & 3.97 & 6.15 & 5.18 \\
         & GPTQ &  6.55 & 5.62 & 4.80 & 4.17 & 6.29 & 5.42 & 3.85 & 5.83 & 4.75 \\
         & AWQ &  6.46 & 5.51 & 4.63 & 3.99 & 6.24 & 5.32 & -  \\
         & OmniQuant  & 6.15 & 5.44 & 4.56 & 3.94 & 6.03 & 5.28 & 3.78 \\ 
          & \cellcolor{Gray}\textbf{GPTVQ 1D (ours)} 
      & \cellcolor{Gray} 6.60
      & \cellcolor{Gray} \textbf{5.34}
      & \cellcolor{Gray} \textbf{4.48}
      & \cellcolor{Gray} \textbf{3.85}
      & \cellcolor{Gray} \textbf{5.97}
      & \cellcolor{Gray} \textbf{5.17}
      & \cellcolor{Gray} \textbf{3.62}
      & \cellcolor{Gray} \textbf{5.76}
            & \cellcolor{Gray} \\
          & \cellcolor{Gray}\textbf{GPTVQ 2D (ours)} 
      & \cellcolor{Gray} \textbf{6.32}
      & \cellcolor{Gray} \textbf{5.31}
      & \cellcolor{Gray} \textbf{4.38}
      & \cellcolor{Gray} \textbf{3.79}
      & \cellcolor{Gray} \textbf{5.82}
      & \cellcolor{Gray} \textbf{5.10}
      & \cellcolor{Gray} \textbf{3.55}
      & \cellcolor{Gray} \textbf{5.51}
            & \cellcolor{Gray} \\
         \midrule
         % \multirow{5}{*}{\shortstack{W4A16}} & RTN & 6.43 & 5.55 & 4.57 & 3.87 & 6.11 & 5.20 & 3.67 \\
         % & GPTQ & 6.13 & 5.40 & 4.48 & 3.83 & 5.83 & 5.13 & 3.58 \\
         % & AWQ &  6.08 & 5.34 & 4.39 & 3.76  & 6.15 & 5.12 & - \\
         % & OmniQuant & 5.86} & 5.21} & 4.25} & 3.71} & 5.74}  & 5.02} & 3.47}  \\ 
         % \hline
         \multirow{6}{*}{\shortstack{4.125 bpv\\(W4@g128)}} & RTN & 5.96 & 5.25 & 4.23 & 3.67 & 5.72 & 4.98 & 3.46  & 5.42 & 4.14\\
         & GPTQ & 5.85 & 5.20 & 4.23 & 3.65 & 5.61 & 4.98 & 3.42 & 5.35 & 4.12 \\
         & AWQ & 5.81 & 5.20 & 4.21 & 3.62 & 5.62 & 4.97 & - \\
         & OmniQuant & \textbf{5.77} & 5.17 & 4.19 & 3.62 & \textbf{5.58} & \textbf{4.95} & 3.40\\
          & \cellcolor{Gray}\textbf{GPTVQ 1D (ours)} 
      & \cellcolor{Gray} 5.96
      & \cellcolor{Gray} \textbf{5.15}
      & \cellcolor{Gray} \textbf{4.18}
      & \cellcolor{Gray} \textbf{3.60}
      & \cellcolor{Gray} 5.61
      & \cellcolor{Gray} \textbf{4.95}
      & \cellcolor{Gray} \textbf{3.38}
      & \cellcolor{Gray} \textbf{5.32}
            & \cellcolor{Gray} \\
          & \cellcolor{Gray}\textbf{GPTVQ 2D (ours)} 
      & \cellcolor{Gray} 5.94
      & \cellcolor{Gray} 5.20
      & \cellcolor{Gray} \textbf{4.18}
      & \cellcolor{Gray} 3.64
      & \cellcolor{Gray} 5.68
      & \cellcolor{Gray} 4.97
      & \cellcolor{Gray} \textbf{3.39}
      & \cellcolor{Gray} 5.44
            & \cellcolor{Gray} \\
        \bottomrule
    \end{tabular}
    %\label{tab:llama_weight_only}
\end{table*}

==> tables/rebuttal_tables_2_3.tex <==
% 
%
\begin{table*}[t]
    \setlength{\tabcolsep}{6pt}
    \centering
    \caption{ \u{Extra weight-only quantization results for {\llama}-2 7B}. We report WikiText-2 (`WT-2') test set perplexity and average zero-shot accuracy of 6 tasks. Numbers marked in bold are SOTA.  
    \emph{Left:} 2-bit weight quantization results. {\ts{\S}}Uses asymmetric weight quantization.
    \emph{Right:} A comparison of the proposed method ($\dcfn{} = {\text{\nf{Q4.4}}}$) with the full-model QAT with W4 and W3 per-channel quantization.}
    % 
    \resizebox{1\columnwidth}{!}{%
    \begin{tabular}{ lcccc }
        \toprule
        % 
        \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{WikiText-2 $\da$} & \multicolumn{2}{c}{Zero-shot acc. $\ua$} \\[0.1em]
        & W2\,pc & W2\,g128 & W2\,pc & W2\,g128 \\
        % 
        \midrule
        % 
        FP16 & \multicolumn{2}{c}{5.68} & \multicolumn{2}{c}{69.68} \\
        \midrule
        RTN\ts{\S} & 5.2e3 & 2.5e3 & 36.52 & 37.94 \\
        GPTQ\ts{\S} & 7.7e3 & 36.77 & - & - \\
        AWQ & - & 2.2e5 & - & - \\
        OmniQuant\ts{\S} & 37.37 & 11.06 & - & - \\
        PEQA\ts{\S} & 9.34 & {7.87} & 57.40 & {60.74} \\
        \gcb{\method{} (ours)}\ts{\S} & \gcb{8.51} & \gcb{7.62} & \gcb{60.03} & \gcb{61.70} \\
        % 
        \bottomrule
    \end{tabular}
        % \vspace{-.15cm}
    % }  % end resizebox

    \,\,\,
    
    % \resizebox{0.3\columnwidth}{!}{%
    \begin{tabular}{ clcc }
        \toprule
        % 
        {\# Bits} & {Method} & {WT-2 $\da$} & {Zero-shot $\ua$} \\ 
        %  
        \midrule
        % 
        \multirow{2}{*}{\shortstack{W4\,pc}} & Full-model QAT & 5.76 & 68.71 \\
        & \gcb{LR-QAT (ours)} & \gcb{5.66} & \gcb{69.95} \\
        % 
        \midrule
        % 
        \multirow{2}{*}{\shortstack{W3\,pc}} & Full-model QAT & 6.14 & 66.91 \\
        & \gcb{LR-QAT (ours)} & \gcb{6.13} & \gcb{67.66} \\
        % 
        \bottomrule
    \end{tabular}
        % \vspace{-.15cm}
    }  % end resizebox    
    \vspace{-.2cm}
\end{table*}
% 



==> tables_and_figures/_04_ablations_prev.tex <==
\begin{table*}[t]
\begin{floatrow}

    

% 
% \begin{figure*}[tb]
%     % \vspace{-.2cm}
%     \includegraphics[width=0.5\textwidth]{}
%     \caption{}
%     \label{fig:04_ablation_rank}
% \end{figure*}
% 
    
    % \hspace{-3pt}
    \includegraphics[width=0.288\textwidth]{img/04_ablation_rank.png}
    % 
    \hspace{0.02\textwidth}
    % 
    % \caption{%
    % A schematic illustration of the attention layer in BERT. 
    % Hidden activation tensor is denoted by $\v{x}$.
    % A problematic residual connection sum after feed-forward network is highlighted in red.
    % }
    % }

    \capbtabbox{%
        \resizebox{0.66\textwidth}{!}{%
        \begin{tabular}{ lllcccc }
            \toprule
            % 
            \multirow{2}{*}{$\dcfn\!\p{\cdot}$} & \multirow{2}{*}{dtype} & \multirow{2}{*}{$\A$, $\B$ init.} & \multicolumn{2}{c}{W4pc} & \multicolumn{2}{c}{W3pc} \\
            & & & WT-2 $\da$ & zero-shot $\ua$ & WT-2 $\da$ & zero-shot $\ua$  \\
            % 
            \midrule
            % 
            {\nf{FP32}} & {\nf{FP32}} & LoRA & 5.69 & 69.28 & 6.21 & 66.62 \\
            \midrule
            {\nf{FP16}} & {\nf{FP32}} & LoRA & $+$0.00 & $-$0.13 & \u{$+$0.01} & $-$0.01 \\
            {\nf{BF16}} & {\nf{FP32}} & LoRA & \u{$-$0.01} & $+$0.11 & \u{$+$0.01} & \u{$+$0.45} \\
            {\nf{Q4.4} / \nf{Q3.5}} & {\nf{FP32}} & LoRA & \u{$-$0.01} & \u{$+$0.16} & \u{$+$0.01} & $+$0.31 \\
            \gcb{\nf{Q4.4} / \nf{Q3.5}} & \gcb{\nf{BF16}} & \gcb{LoRA} & \gcb{$-$0.01} & \gc{$+$0.15} & \gcb{$+$0.01} & \gc{$+$0.31} \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoRA & $+$0.02 & $-$0.04 & $+$1.5e3 & $-$30.30 \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoftQ ($T=1$) & $+$0.14 & $-$1.02 & $+$0.18 & $+$0.26 \\
            {\nf{INT-4} / \nf{INT-3}} & {\nf{FP32}} & LoftQ ($T=64$) & $+$0.40 & $-$1.40 & $+$1.37 & $-$2.01 \\
            % 
            \bottomrule
        \end{tabular}
        } % // end resizebox
        % \vspace{-.15cm}
    % \centering
    % \ffigbox[\FBwidth]{
    }  %// end capbtabbox
    
    \captionlistentry[figure]{}
    \label{fig:04_ablation_rank}
    \vspace{-.1cm}
    \captionsetup{labelformat=andfigure}
    \caption{%
    \emph{Left}: The performance of {\method} ($\dcfn{} = {\text{\nf{Q4.4}}}$) depending on the rank $r$ of auxiliary matrices $\A$ and $\B$ on {\llama}-2 7B with W4 per-channel quantization.
    % 
    We report mean and standard deviation over 5 runs with different random seeds.
    % 
    \emph{Right}: The performance of {\method} applied to {\llama}-2 7B depending on the choice of downcasting operator $\dcfn\!\p{\cdot}$, compute data type, and initialization method for low-rank auxiliary matrices.
    % 
    We report WikiText-2 (`WT-2') test set perplexity, lower is better, and average zero-shot accuracy of 6 tasks, higher is better.
    % 
    Numbers marked in bold are the best results.
    }
    \label{tbl:04_ablation_dtype_init}
\end{floatrow}
\vspace{-.1cm}
\end{table*}


==> tables_and_figures/_archive/_tmp.tex <==
\begin{table*}[ht]
\begin{floatrow}

    \capbtabbox{%
    \begin{tabular}{ lcccc }
        \toprule
         Quantized activations & STS-B & MNLI & QNLI & RTE \\
         \midrule  
         none (FP32 model) & 89.09 & 84.91 & 91.58 & 70.40 \\
         all & 62.64	&	42.67	&	50.74	&	48.74	\\
         \midrule  
         all, except softmax input & 70.92	&	42.54	&	51.84	&	48.74	\\
         all, except sum of embeddings & 67.57	&	46.82	&	51.22	&	51.26	\\
         all, except self-attention output & 70.47	&	46.57	&	50.98	& 50.90 \\
         all, except softmax output & 72.83	&	50.35	&	50.23	&	49.46	\\
         all, except residual connections after FFN & \bf{81.57}	&	\bf{82.56}	&	\bf{89.73}	&	\bf{67.15}	\\
         same as above, but for layers 10, 11 only & \bf{79.40}	&	\bf{81.24}	&	\bf{88.03}	&	\bf{63.90}	\\
         \bottomrule
    \end{tabular}
    % \caption{Leave-one-out analysis for activation quantizers.}
    }

    % \centering
    % \ffigbox[\FBwidth]{
    \hspace{-3pt}
    \includegraphics[width=0.19\textwidth]{figures/03_residual_connections_ffn_no_border_v5}
    \hspace{-6pt}
    % \caption{%
    % A schematic illustration of the attention layer in BERT. 
    % Hidden activation tensor is denoted by $\v{x}$.
    % A problematic residual connection sum after feed-forward network is highlighted in red.
    % }
    % }
    
    \captionlistentry[figure]{}
    \label{fig:03_attention_layer}
    \captionsetup{labelformat=andfigure}
    \caption{%
    \emph{Left}: Leave-one-out analysis for activation quantizers on problematic GLUE tasks.
    We set all weights to FP32 and use current min-max (with a batch size of 1) range estimator for activations. 
    We report median score over 5 runs with different random seeds.
    \emph{Right}: A schematic illustration of the attention layer in BERT. 
    Hidden activation tensor is denoted by $\v{x}$. $\oplus$ is an element-wise addition.
    A problematic residual connection sum after feed-forward network is highlighted in red.
    }
    \label{tbl:03_loo_analysis}
\end{floatrow}
\end{table*}

